Elliptical Slice Sampling for Probabilistic Verification of Stochastic Systems with Signal Temporal Logic Specifications

Autonomous robots typically incorporate complex sensors in their decision-making and control loops. These sensors, such as cameras and Lidars, have imperfections in their sensing and are influenced by environmental conditions. In this paper, we present a method for probabilistic verification of linearizable systems with Gaussian and Gaussian mixture noise models (e.g. from perception modules, machine learning components). We compute the probabilities of task satisfaction under Signal Temporal Logic (STL) specifications, using its robustness semantics, with a Markov Chain Monte-Carlo slice sampler. As opposed to other techniques, our method avoids over-approximations and double-counting of failure events. Central to our approach is a method for efficient and rejection-free sampling of signals from a Gaussian distribution such that satisfy or violate a given STL formula. We show illustrative examples from applications in robot motion planning.

==> outline.tex <==
\section{Outline}


\begin{enumerate}
    \item more accurate than chance constraints
    \item Single gaussian noise 
    \begin{itemize}
        \item compare to MC - computation is better
        \item feedback regarding reason for failure
    \end{itemize}
    \item complex noise
        \begin{itemize}
        \item still works
         \item compare to MC - computation is worse
        \item feedback is better - connection to noise
    \end{itemize}
    \item useful for feedback to designer and for later synthesis
\end{enumerate}
\begin{enumerate}
    \item Introduction:
    \begin{enumerate}
        \item Motivation in the sense of examples where we show that system with perception have more intricate noise models than Gaussians and it affects the closed loop system (beam model, system with ML component, the car-following controller, dropouts, adversarial affecting the sensors etc...). And, how we're able to compute the probability of satisfying/falsifying an STL specification (complex tasks, adding reachability to the always avoid option).
        \item Work done with chance constraints and why it is not good enough (double counting, bounds are too loose etc...). 
        \item Work done with Monte-Carlo techniques, even those that are directed, why and in what cases it is slow.
        \item The new elliptical slicing technique we are basing our approach on.
    \end{enumerate}
    \item Preliminaries:
    \begin{enumerate}
        \item Mathematical intro to the elliptical slicing and HDR algo from the other paper.
        \item STL in a nutshell
    \end{enumerate}
    \item Problem setup:
    \begin{enumerate}
        \item The system and assumptions (linear, Gaussian noises ...)
        \item The noise model (Gaussian Mixture, and the mixands could be sampled from some fixed distribution (Bernoulli) or from a Markov Chain model and we motivate why it is a possible good model for modeling complicated events.
    \end{enumerate} 
    \item Approach:
    \begin{enumerate}
        \item Overview: sampling modes, getting trajectories
        \item Generate the trajectory distribution (noises to trajectories)
        \item How we model the regions in the specs and in time, the horizon etc.
        \item How much noise modes do we need to sample (variance of the p(fail) when sampling a trajectory) and the confidence interval for our computation.
        \item How do we overcome the intervals between two points that come from discretization.
    \end{enumerate} 
    \item Examples:
    \begin{enumerate}
        \item Holonomic 2-D robot trying to reach a goal within time limits while avoiding obstacles in an STL specification.
        \item A more complex robotic manipulator doing the same thing in a more complex environment.
        \item Comparisons to a naive Monte-Carlo
    \end{enumerate}
    \item \sout{Synthesis (optional):} 
    \begin{enumerate}
        \item Using the derivative feature of the method in order to drive the $\mu$ or $\Sigma$ (and even better - the reference commands or the controller parameters) in such a way that the p(fail) would decrease. 
        \item Using the sampler to find its own trajectories the satisfy the specifications. Once the algorithm succeeds, it is easy to sample from those trajectories so essentially we have a policy to use. The problem is finding the first trajectory that is within a specifying set.
    \end{enumerate}
    \item Discussion
\end{enumerate}

\textbf{Main contributions:}
\begin{enumerate}
    \item Computation framework to accurately compute the probability of a system to satisfy an STL specification (of course it can also be just some environment with obstacles and a nominal trajectory to execute).
    \item The probabilities of failure are not counted twice, are not overapproximated and are efficiently solved (and can even be parallelized). 
    \item Deal with more intricate noises that can express more involved modeling options, and not just Gaussians.
    \item Able to sample from the trajectories that are failing/succeeding - for analysis purposes, for ...?
    \item \sout{Synthesis (if available) - change the parameters of the system via gradient decent such that the probability of failure decreases with respect to the complex noise model.}
\end{enumerate}

